Optimal Collaborative Transportation for Under-Capacitated Vehicle Routing Problems using Aerial Drone Swarms

Swarms of aerial drones have recently been considered for last-mile deliveries in urban logistics or automated construction. At the same time, collaborative transportation of payloads by multiple drones is another important area of recent research. However, efficient coordination algorithms for collaborative transportation of many payloads by many drones remain to be considered. In this work, we formulate the collaborative transportation of payloads by a swarm of drones as a novel, under-capacitated generalization of vehicle routing problems (VRP), which may also be of separate interest. In contrast to standard VRP and capacitated VRP, we must additionally consider waiting times for payloads lifted cooperatively by multiple drones, and the corresponding coordination. Algorithmically, we provide a solution encoding that avoids deadlocks and formulate an appropriate alternating minimization scheme to solve the problem. On the hardware side, we integrate our algorithms with collision avoidance and drone controllers. The approach and the impact of the system integration are successfully verified empirically, both on a swarm of real nano-quadcopters and for large swarms in simulation. Overall, we provide a framework for collaborative transportation with aerial drone swarms, that uses only as many drones as necessary for the transportation of any single payload.

==> contents/images/algorithms_flowchart.tex <==
\usetikzlibrary{shapes,arrows}

\begin{tikzpicture}[node distance=2cm, auto]
    % Define styles for nodes
    \tikzstyle{block} = [rectangle, draw, text width=6em, text centered, minimum height=3em]
    \tikzstyle{circleblock} = [ellipse, draw, text width=6em, text centered, minimum height=3em]
    \tikzstyle{line} = [draw, {Latex[length=4mm,width=60mm]}, line width=1pt]

    % Nodes
    \node [circleblock] (problem) {Problem Statement};
    \node [block, right of=problem, xshift=2cm] (solver) {cmTSP Solver};
    \node [block, below of=problem, xshift=2cm] (solution) {Solution (Mission Matrix)};
    \node [block, below left of=solution, xshift=-1cm] (path) {Path Planner};
    \node [block, below right of=solution, xshift=1cm] (scheduler) {Mission Scheduler};
    \node [block, below of=solution, yshift=-1.5cm] (controller) {Drones Controller};

    % Arrows
    \path [draw, -latex'] (problem) -- (solver);
    \path [draw, -latex'] (solver) |- (solution.east);
    \path [draw, -latex'] (solution.west) -| (path.north);
    \path [draw, -latex'] (solution.east) -| (scheduler.north);
    \path [draw, -latex'] (path) -- (controller);
    \path [draw, -latex'] (scheduler) -- (controller);
    \path [draw, latex'-latex'] (path) -- (scheduler);

\end{tikzpicture}

